Challenging theories of gravitation: dark matter, compact objects and gravitational waves

The most accurate model to describe the gravitational interaction is the well-known theory of General Relativity. Several observational evidences corroborate the legitimacy of the theory compared to the older Newtonian gravity. General Relativity furthermore predicts the existence of gravitational waves, i.e. spacetime ripples produced by accelerated masses. Thanks to a connected network of interferometers called LIGO/Virgo, gravitational waves from the coalescence of massive and compact astrophysical bodies have been measured directly. These recent observations paved the way to a completely new route to test the gravitational interaction. The possibility of using gravitational waves to obtain a deeper understanding of open problems within General Relativity motivates the work developed in this thesis. Each part is essentially devoted to challenging the current model of gravitation, sometimes including yet undiscovered new matter fields, and other times modifying the theoretical framework of General Relativity. In the first part of this manuscript, I discuss the astrophysical consequences of the presence of scalar fields permeating galaxies. A detailed picture of the interaction of massive black holes and scalar dark matter structures is provided. The second part is dedicated to the analysis of the generation and propagation of gravitational waves. As an example, I examine the close limit approximation as a promising tool to investigate the collision of extreme compact objects. The last part of this thesis instead focuses on unstable mechanisms around black holes and stars (scalarization and vectorization), in two alternative models of gravitation.

==> Intro_on_GW.tex <==
\chapter{Basic concepts of gravitational wave physics}

==> app_clap.tex <==
\chapter{Initial data for the interior of an Extreme Compact Object}\label{app:ECO_initialdata}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We shall model the ECO interior, finding (in the framework of a $3+1$ decomposition, see Sec.~\ref{sec:3+1}) a
conformally flat three-metric
%
\begin{equation}
\prescript{3}{}{ds}^2_{\rm ECO}=\varphi^4 \prescript{3}{}{d\eta}^2=\varphi^4 \left( dR^2+R^2d\Omega^2 \right)\,,
\label{eq:ds2ECO}
\end{equation}
%
solution of the Hamiltonian constraint equation~\eqref{eq:H_ECO}, which, with the ansatz~\eqref{eq:ds2ECO}, can
be written as
%
\begin{equation} \label{eq:ECO_Hamiltonian_constraint}
\nabla^2_{\eta}\varphi=-2\pi \rho \varphi^{5}\,.
\end{equation}
%
We shall first consider a single, static ECO; then, we shall consider two close static ECOs at rest. Our solution can,
in principle, be matched with the BL solution in the exterior discussed in Sec.~\ref{subsec:BL-ECO}, where $R$ is the
isotropic coordinate defined in Eq.~\eqref{eq:R_isotropic_to_ECO}. The interior solution is defined for $R\le R_0$,
where $R=R_0$ is the ECO surface. 

We shall consider, for a single, static ECO, a density profile of the form
\begin{equation}
\rho=\frac{\varphi^{-5}}{2\pi}\left[
\frac{3 M}{2R_0^3}\Theta\left( R_0-R\right)  \right]\,.\label{eq:ECOrho}
\end{equation}
%
Therefore, Eq.~\eqref{eq:ECO_Hamiltonian_constraint} gives, 
%
\begin{equation}
  \nabla^2_{\eta}\varphi=
  \frac{3M}{2R_0^3}  \Theta\left( R_0-R\right)\,.\label{eq:phi_ECO}
\end{equation}
%
This choice can be considered either as a toy model, or as a specific example of an ECO interior. We stress that the
interior structure of the ECO does not enter in the GW signal computed in this article, since we assume that --~due to
the small lapse~-- the internal degrees of freedom do not significantly affect the GW emission and thus can safely be
neglected (see Sec.~\ref{subsec:BL-ECO}).

The exterior solution (i.e. Schwarzschild's metric) for $R\ge R_0$ is $\varphi=1+M/(2R)$. 
The solution of Eq.~\eqref{eq:phi_ECO} matching with the exterior is
%
\begin{equation}
\varphi=1+\frac{M}{2}\left( \frac{3}{2R_0}-\frac{R^2}{2R_0^3}\right)+\frac{M}{2}\left( \frac{1}{R}+\frac{R^2}{2R_0^3}-\frac{3}{2R_0}\right) \Theta\left( R-R_0\right)\,.
\end{equation}
%
Let us now consider two ECOs at rest, with the same positions as the BHs in the BL initial data (see
Sec.~\ref{subsec:BL}), $(0,0,\pm Z_0)$, having radii $\widetilde{R}_1$, $\widetilde{R}_2$, and ``bare'' masses $m_1$,
$m_2$, corresponding to the ADM masses (see Sec.~\ref{subsec:BL-ECO}) $M_1=m_1(1+m_2/(4Z_0))$, $M_2=m_2(1+m_1/(4Z_0))$;
the ADM mass of the final object is $M=m_1+m_2$.

%We shall assume that the
%two ECOs do not intersect, thus $d=R_1+R_2>2R_0$.
%In Sec.~\eqref{sec:BH_mimickers} we consider, in particular, the case $M_1=M_2=M/2$
%If $R_1=R_2=Z_0/2$ and $R_0\simeq M/2$, this implies that $Z_0/M\gtrsim0.5$. \leo{Do you agree with this bound? If $Z_0/M<0.5$ the  ECOs touch. We should say this also in the body of the text}
 
%The density profile is then
%\begin{align}
%\rho(X,Y,Z)=&\frac{\varphi^{-5}}{2\pi}\left[
%  \frac{3 M_1}{2R_1^3}\Theta(R_1-\sqrt{X^2+Y^2+(Z+Z_0)^2})\right.\nonumber\\
%  &\left.+\frac{3 M_2}{2R_2^3}\Theta(R_2-\sqrt{X^2+Y^2+(Z-Z_0)^2})
%\right]
%\end{align}
The constraint equation has the form 
\begin{equation}
 \nabla^2_{\eta}\varphi=
  -\frac{3 m_1}{2R_1^3}\Theta(\widetilde{R}_1-\sqrt{\Delta-2Z_0R\cos\theta})-\frac{3 m_2}{2R_2^3}\Theta(\widetilde{R}_2-\sqrt{\Delta+2Z_0R\cos\theta})\,,\label{eq:equationBECO}
\end{equation}
where $\Delta=R^2+Z_0^2$ and $\cos\theta=Z/R$.
Matching with the BL solution~\eqref{eq:BL_id_newtonian} gives:
%
\begin{equation}
\varphi=1-\frac{m_1}{2}\Upsilon\left( \widetilde{R}_1\right)-\frac{m_2}{2}\Upsilon\left( \widetilde{R}_2\right)+\frac{R Z_0 \cos\theta}{2}\left[\frac{m_1}{\widetilde{R}_1^3}-\frac{m_2}{\widetilde{R}_2^3} \right]
  +\frac{m_1 g_{\left( \widetilde{R}_1,Z_0\right)}+m_2 g_{\left( \widetilde{R}_2, -Z_0\right)}}{2}\,,
\end{equation}
where
\begin{align}
\Upsilon\left( \widetilde{R}_i\right)&=\frac{R^2+Z_0^2-3\widetilde{R}_i^2}{2\widetilde{R}_i^3}\nn\\
\label{eq:upsilon_and_g}
g_{\left( \widetilde{R}_i,Z_0\right)}&=\Bigg[\frac{1}{\sqrt{\Delta+2 Z_0 R \cos\theta}} -\frac{3}{2\widetilde{R}_i} +
  \frac{\Delta+2 Z_0 R \cos\theta}{2\widetilde{R}_i^3} \Bigg]\Theta\left[ \sqrt{\Delta+2 Z_0 R \cos\theta}-\widetilde{R}_i \right]\,.
\end{align}
%
For an equal mass binary ECO ($m_1=m_2=M/2$, $R_1=R_2=R_0$), the conformal factor reduces to  
%
\begin{equation} \label{eq:id_ECOs_equalmasses}
\varphi= 1-\frac{M}{2}\Upsilon\left( R_0\right) +\frac{M}{4} \left[ g_{\left( R_0,Z_0\right)}+ g_{\left( R_0, -Z_0\right)}\right]\,,
\end{equation}
%
with $\Upsilon$ and $g$ defined in Eq.~\eqref{eq:upsilon_and_g}. An example of this configuration is represented in
Fig.~\ref{fig:BECO_initialvalue} for various ECOs distances.

We remark that this solution has been determined under the assumption that the two ECOs do not overlap, i.e. that
$Z_0>R_0$. Since (for $\epsilon\ll1$) $R_0\simeq M/2$, this implies that $Z_0/M\gtrsim0.5$. When the ECOs overlap, the
solution~\eqref{eq:id_ECOs_equalmasses} should be considered as a rough approximation. We remark, however, that the
model of the interior does not affect the GW signal derived in Sec.~\ref{subsec:ECO-collision}, because the internal
degrees of freedom are, with good approximation, decoupled from the evolution of the exterior spacetime.
%
\begin{figure}[ht]
\centering
\includegraphics[width=0.7\textwidth,keepaspectratio]{Plots/BBHM_initialdata.png}
\caption{Curves with the same value of $\varphi$ for an equal mass binary ECO spacetime ($m_1=m_2=M/2$,
  $R_1=R_2=R_0$). The axes are normalized to the mass of the final ECO ($Y/M, Z/M$), and each frame represents a $Y-Z$
  spatial slice of the conformal factor. Starting from the upper-left panel and moving clockwise in the panels, ECOs are
  at a distance $Z_0=M\{1/4,3/4,1,2\}$ from the origin of the reference frame. The dashed red circles corresponds to the
  colliding ECOs surfaces and the solid green one to the final static ECO.  }
%
\label{fig:BECO_initialvalue}
\end{figure}
%





==> app_clap_KG.tex <==
\chapter{Perturbative expansion of the Klein-Gordon equation}\label{app:separateKG}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Let us consider the Klein-Gordon equation for a massless scalar field,
\begin{equation}
\square\Phi=\frac{1}{\sqrt{-g}}\partial_\mu\left(g^{\mu\nu}\sqrt{-g}\partial_\nu\right)\Phi=0
\end{equation}
on the binary BH spacetime described by the BL solution linearized in the quadrupole contribution,
$g_{\mu\nu}=g^{(0)}_{\mu\nu}+h_{\mu\nu}$ with $g^{(0)}_{\mu\nu}$ Schwarzschild metric and $h_{\mu\nu}$ given in
Eq.~\eqref{eq:BLrecast1}. Expanding the D'Alambertian operator in powers of the parameter $Z_0$ as in
Eq.~\eqref{eq:box_expansion}, neglecting the terms $O(Z_0^3)$, it has the form:
%
\begin{equation} \label{eq:KG_pert}
\left( \square^{(0)}+ Z_0^2 \, \square^{(1)} \right) \Phi =0\,.
\end{equation}
%
We expand the scalar field in scalar spherical harmonics $Y^{\ell m}(\theta,\phi)$, as in
Eq.~\eqref{eq:spher_harm_decomp}. Since Schwarzschild's spacetime is spherically symmetric, the spherical harmonics are
eigenfuctions of the the D'Alambertian on $g^{(0)}_{\mu\nu}$, $\square^{(0)}$, while the operator $\square^{(1)}$
couples harmonics with different values of $\ell$ (but do not couple harmonics with different values of $m$).

We shall look for a solution which, in the limit $Z_0\to0$, has given harmonic indexes $(\ell,m)$. The contributions
with $\ell'\neq\ell$ are of order $O(Z_0^2)$, and we can write
\begin{equation} \label{eq:Phi_ansatz_2}
\Phi=\frac{\psi_{\ell\,m}\left( t,r\right) Y^{\ell\,m}\left(\theta,\phi\right)}{r}+Z_0^2 \sum_{\ell'\neq\ell}\frac{\psi_{\ell'\, m}\left( t,r\right) Y^{\ell'\, m}\left(\theta,\phi\right)}{r}\,.
\end{equation}
Replacing Eq.\til\eqref{eq:Phi_ansatz_2} in Eq.\til\eqref{eq:KG_pert} we find 
%
\begin{equation} \label{eq:KG_pert_2}
\square^{(0)} \left[\frac{\psi_{\ell\, m} Y^{\ell\,m} \left(\theta,\phi\right)}{r}\right]+ Z_0^2  \square^{(1)} \left[ \frac{\psi_{\ell\,m} Y^{\ell\,m} \left(\theta,\phi\right)}{r} \right]+ Z_0^2 \sum_{\ell'\neq \ell} \square^{(0)} \left[ \frac{\psi_{\ell'\,m} Y^{\ell'\,m} \left(\theta,\phi\right)}{r}\right] =0\,.
\end{equation}
%
Since the spherical harmonics are eigenfunctions of the operator $\square^{(0)}$, by projecting the above equation on
the complete basis of spherical harmonics, the components $\psi_{\ell'\,m}$ with $\ell'\neq\ell$ vanish, and we obtain a
{\it decoupled equation}, whose solution, with appropriate boundary conditions, gives the ``deformed'' QNMs
corresponding to the harmonic indexes $\ell,m$. We note that this result is analogous to the case of slowly rotating
spacetimes, whose QNMs - at leading order in the rotation - are not affected by the couplings between different harmonic
components~\cite{kojima1993normal,Pani:2012bp}. The $O(Z_0^2)$ term of Eq.~\eqref{eq:KG_pert_2} can be written as
\begin{align}
&\square^{(1)} \left[ \frac{\psi_{\ell\,m} Y^{\ell\,m} \left(\theta,\phi\right)}{r} \right]=-\frac{\partial Y^{\ell\, m}}{\partial \theta}\frac{3 g \sin (2 \theta ) }{8 M^2 r^3}\psi_{\ell\,m}\nn\\
&+Y^{\ell\, m}\Bigg(- r\left(-r^2 f dg/dr+4 M g\right)\frac{\partial \psi_{\ell\,m}}{\partial r}-2r^3 f g\frac{\partial^2 \psi_{\ell\,m}}{\partial r^2}\nn\\
&+\left(-r^2 f dg/dr+2 g (\ell (\ell+1) r+2 M)\right)\psi_{\ell\,m}\Bigg)\frac{\alpha\left(\theta\right)\,}{16 M^2 r^4} \,,
\label{eq:KGZ02}
\end{align}
where $\alpha\left(\theta\right)=1+3 \cos (2 \theta )$ and we remind that $f=1-2M/r$. The projection on $Y^{\ell\,m}$ of the $O(0)$ terms in Eq.~\eqref{eq:KG_pert_2} yields the standard scalar field equation in
Schwarzschild spacetime, 
\begin{equation} 
 -\frac{1}{r f}\Bigg(\frac{\partial^2\psi_{\ell\,m}}{\partial t^2}-f^2\frac{\partial^2\psi_{\ell\, m}}{\partial r^2}
  -f\frac{df }{dr}\frac{\partial\psi_{\ell\, m}}{\partial r}+f\frac{\ell (\ell+1) r+2 M }{r^3}\psi_{\ell\, m}\Bigg)\,.
\end{equation}
If we include the projection on $Y^{\ell\,m}$ of the $O(Z_0^2)$ terms, i.e. of
Eq.~\eqref{eq:KGZ02}, Eq.~\eqref{eq:KG_pert_2} gives
%%%%%%%%%%%%%%%%%%%
\begin{equation} \label{eq:KG_notortoise_app}
 \frac{\partial^2 \psi_{\ell\,m}}{\partial t^2}+\frac{\partial^2 \psi_{\ell\,m}}{\partial r^2}
  \left( U_0+Z_0^2\tilde{U}_0\right)+\frac{\partial \psi_{\ell\,m}}{\partial r}  \left( U_1+Z_0^2\tilde{U}_1\right)+\psi_{\ell\,m} \left(  W_0 +Z_0^2  W_1\right)=0\,,
\end{equation}
where 
\begin{align}
\label{eq:potentials_notortoise}
&U_0(r)=-f^2\,,\nn\\
&\tilde{U}_0(r)=\frac{\left( r-2 M \right) f q^{(1)}_{\ell\,m} g}{8M^2r}\,,\nn\\
&U_1(r)= -f \frac{df}{dr} \,,\nn\\
& \tilde{U}_1(r)= -\frac{q^{(1)}_{\ell\,m} (2 M-r) \left(4 M g(r)-f r^2 dg/dr\right)}{16 M^2 r^3}\,,\nn\\
&W_0(r)=f\frac{\ell (\ell+1) r+2 M }{r^3}\,,\nn\\
&W_1(r)=\frac{q^{(1)}_{\ell\,m}}{16 M^2 r^4} (f r^2 (r-2 M) dg/dr\nn\\
&+2 g (2 M-r) (l (l+1) r+2 M))+3q^{(2)}_{\ell\,m}\frac{(r-2M)g}{4M^2r^3}\,,
\end{align}
and we have defined the constant coefficients
%\begin{widetext}
%
%\begin{align}
%  &  Z_0^2\left( \int d\Omega \left( Y^{\ell\,m}\right)^* Y^{\ell\,m} \left( 1+3\cos\left( 2 \theta\right)\right) \right)
%  \frac{1}{8r^4} \Bigg[r \left(\left(r (r-2 M) \frac{1}{2M^2}\frac{dg}{dr}-\frac{2g}{M}\right) \frac{\partial
%      \psi_{\ell\,m}}{\partial r}-\frac{g}{M^2}  r (r-2 M) \frac{\partial^2 \psi_{\ell\,m}}{\partial r^2}\right)\nn\\
%    &+\psi_{\ell\,m} \left( \frac{g}{M^2} (l (l+1) r+2 M)+r (2 M-r) \frac{1}{2M^2}\frac{dg}{dr}\right) \Bigg]- Z_0^2
%  \frac{3 g \psi_{\ell\,m}}{4 M^2 r^3}  \left(\int d\Omega \sin \theta \cos \theta \left( Y^{\ell\,m}\right)^*
%  \frac{d Y^{\ell\,m}}{d\theta}\right)\,.
%\end{align}
%%
%\end{widetext}
%
\begin{align} \label{eq:q1lm}
q^{(1)}_{\ell\,m}  \equiv&\int d\Omega \left( Y^{\ell\,m}\right)^* Y^{\ell\,m} \alpha
  \,,\\ \label{eq:q2lm}
  q^{(2)}_{\ell\,m}\equiv &\int d\Omega \sin \theta \cos \theta \left( Y^{\ell\,m}\right)^*
  \frac{d Y^{\ell\,m}}{d\theta}  \,.
\end{align}
Note that
\begin{equation}
\label{eq:q12lm}
q^{(1)}_{00}=q^{(2)}_{00}=0\,,
\end{equation}
therefore the $\ell=0$ equation is not affected by the $O(Z_0^2)$ corrections. For $0<\ell\le2$, the quantities
$q^{(1,2)}_{\ell\,m}$ are:
\begin{align} 
&  q^{(1)}_{1-1}=q^{(1)}_{11}=-\frac{4}{5},\,q^{(1)}_{10}=\frac{8}{5}\,,\nonumber\\
&  q^{(1)}_{2-2}=q^{(1)}_{22}=-\frac{8}{7},\,q^{(1)}_{2-1}=q^{(1)}_{21}=\frac{4}{7},\,q^{(1)}_{20}=\frac{8}{7}\,,\nonumber\\
& q^{(2)}_{1-1}=q^{(2)}_{11}=\frac{1}{5},\,q^{(2)}_{10}=-\frac{2}{5}\,,\nonumber\\
& q^{(2)}_{2-2}=q^{(2)}_{22}=\frac{2}{7},\,q^{(2)}_{2-1}=q^{(2)}_{21}=-\frac{1}{7},\,q^{(2)}_{20}=-\frac{2}{7}\,.
\end{align}
%



==> app_sphericalBox.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\chapter{Exciting a spherical box} \label{app:internal_modes}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Here we study the scalar field inside a spherical box of radius $R$, which is sourced by a particle in circular orbital motion.
Our approach to study the resonances follows the treatment of forced oscillations in Ref.~\cite{landau1982mechanics}.


Consider a $U(1)$-invariant scalar field theory described by the action
\begin{equation} \label{theory}
	S\equiv \frac{1}{2}\int d^4 x \sqrt{-\eta} \,\partial^\mu \Phi \partial_\mu \Phi^*\,,
\end{equation}
on a Minkowski background. Moreover, let us consider that this scalar field is sourced by a point particle through the action~\eqref{coupling_Qball}. 
Let us first start with the sourced equation of motion
\begin{equation}\label{eq:box}
	\nabla_\mu\partial^\mu  \Phi= T_p\,,
\end{equation}
which is obtained through the variation of the total action, and where $T_p$ is the trace of the particle's stress-energy tensor. Assuming the particle motion to be in the equatorial plane, with $r_{\rm orb}$ and $\omega_{\rm orb}$, the orbital radius and angular frequency, respectively, the trace of the particle's stress-energy tensor is given by Eq.~\eqref{T_p_orbiting}. Consider then the decompositions
\begin{align*}
	\Phi&=\sum_{l,m}\int \frac{d\omega}{\sqrt{2\pi}}e^{-i\omega t}\frac{\phi(r;\omega,l,m)}{r}Y_{l}^m(\theta,\varphi)\,, \\
	T_p&=\sum_{l,m}\int \frac{d\omega}{\sqrt{2\pi}}e^{-i\omega t}\frac{T_{l}^m(r;\omega)}{r^2}Y_{l}^m(\theta,\varphi) \,.
\end{align*}
Thus, one can use the method of variation of parameters to obtain the general inhomogeneous solution of Eq.~\eqref{eq:box}
%
\begin{equation}
\phi=\phi^h-\phi^I \int_0^r dr'\left(\frac{\phi^{II} T_l^m}{r' W}\right)-\phi^{II} \int_r^R dr'\left(\frac{\phi^{I} T_l^m}{r' W}\right)\,,\nonumber
\end{equation}
with $0 \leq r\leq R$, where $\phi^h$ is the general homogeneous solution
\begin{equation*}
	\phi^h=A_I \phi^I+A_{II} \phi^{II}\,,
\end{equation*}
with
\begin{align*}
\phi^I&=\sqrt{r} \left[J_{l+\frac{1}{2}}(\omega r)-\frac{J_{l+\frac{1}{2}}(\omega R)}{Y_{l+\frac{1}{2}}(\omega R)}Y_{l+\frac{1}{2}}(\omega r)\right]\,,\\
\phi^{II}&=\sqrt{r} J_{l+\frac{1}{2}}(\omega r)\,.
\end{align*}
%
The Wronskian of $\phi^I$ and $\phi^{II}$ is $W=2 J_{l+\frac{1}{2}}(\omega R)/\left(\pi Y_{l+\frac{1}{2}}(\omega R)\right)$. 

Now, we want to impose regularity at the origin $\phi(0)=0$, and Dirichlet conditions at the surface of the box $\phi(R)=0$. Notice that the homogeneous solutions $\phi^{II}$ satisfy these boundary conditions for discrete values of $\omega=\omega_n$ (with $n \in \mathbb{Z} \setminus \{0\}$), such that $J_{l+\frac{1}{2}}(\omega_n R)=0$; the frequencies $\omega_n$ are the normal modes of a scalar field in a spherical box. The wronskian above vanishes for these modes. We use the notation $\omega_{-n}=-\omega_n$.

For $\omega \neq \omega_n$, the boundary conditions imply that $\phi^h=0$. Thus,
%
\begin{equation}
\phi=A_l^m(\omega) \phi^{II} \delta(\omega-\omega_n)-\phi^I \int_0^r dr'\left(\frac{\phi^{II} T_l^m}{r' W}\right)-\phi^{II} \int_r^R dr'\left(\frac{\phi^{I} T_l^m}{r' W}\right)\,,\nonumber
\end{equation}
%
with arbitrary complex coefficients $A_l^m(\omega_n)=A_{l,n}^m$.
In particular, at the origin,
%
\begin{equation} 
\phi(r\to 0)\sim\left(\frac{\omega}{2}\right)^{l+\frac{1}{2}} \frac{r^{l+1}}{\Gamma\left(l+\frac{3}{2}\right)} \left[A_l^m(\omega) \delta(\omega-\omega_n)-\int_0^R dr'\left(\frac{\phi^{I} T_l^m}{r' W}\right)\right]\,.\nonumber
\end{equation}
%
The total field at the origin is then
%
\begin{align}
	\Phi(r\to 0)&\sim \sum_{l,m}\frac{ Y_l^m(\theta,\varphi)r^{l}}{\Gamma\left(l+\frac{3}{2}\right)2^{l+\frac{1}{2}}} \left[\sum_{n \neq 0}\frac{(\omega_n)^{l+\frac{1}{2}}}{\sqrt{2\pi}} A_{l,n}^me^{-i\omega_n t}+ \right. \nonumber \\
	&\left. m_p(m \omega_{\rm orb})^{l+\frac{1}{2}} \sqrt{1-(r_{\rm orb} \omega_{\rm orb})^2} Y_l^m\left(\frac{\pi}{2},0\right) \frac{\phi^I e^{-i m \omega_{\rm orb} t}}{r_0 W(m\omega_{\rm orb})} \right]\,,\nonumber
\end{align}
%
with $\phi^I=\phi^I(r_{\rm orb}; m \omega_{\rm orb})$.
For simplicity, take for now $A_{l,n}^m=0$ (\textit{i.e.} we neglect the free normal mode part of the solution).
Moreover, notice that in this theory the energy density of the scalar field is
%
\begin{equation}
	T_{t t}=\frac{1}{2}\left(|\partial_t \Phi|^2+|\partial_r \Phi|^2+\frac{1}{r^2} |\partial_\theta \Phi|^2 +\frac{1}{r^2 \sin^2 \theta} |\partial_\varphi \Phi|^2\right)\,.\nonumber
\end{equation}
%
Thus, at the origin, the energy density is
%
\begin{equation}
T_{t t}(0)\sim	\frac{\omega_{\rm orb}^3}{16 \pi^3}\left(\frac{m_p \phi^I(r_{\rm orb};\omega_{\rm orb})}{r_{\rm orb}W(\omega_{\rm orb})}\right)^2\left[1-\left(r_{\rm orb} \omega_{\rm orb}\right)^2\right]\,.\nonumber
\end{equation}
%
Since the Wronskian $W$ vanishes for $\omega_{\rm orb}=\omega_{n'}$, the energy density $T_{t t}(r\to 0)$ diverges for these frequencies. Thus, resonances are produced for particles with orbital frequencies $\omega_{\rm orb}=\omega_{n'}$. 

It is interesting to pose the question of how $T_{t t}(r\to 0)$ increases with time when the system is in resonance with $\omega_{\rm orb}=\omega_{n'}$. To answer this, let us choose
%
\begin{equation}
A_{l,n}^m=-\sqrt{2 \pi} m_p \sqrt{1-(r_{\rm orb} \omega_{\rm orb})^2}(1-\delta_0^m)\delta_n^{\text{sign}(m)\,n'} Y_l^m\left(\frac{\pi}{2},0\right) \frac{\phi^I(r_{\rm orb}; m \omega_{\rm orb})}{r_{\rm orb} W(m\omega_{\rm orb})}\left(\frac{m \omega_{\rm orb}}{\omega_n}\right)^{l+\frac{1}{2}}.\nonumber
\end{equation}
%
With this choice, the total field at the origin is
%
\begin{align}
\Phi&\sim \sum_{l,m\neq 0}\frac{ Y_l^m(\theta,\varphi)r^{l}}{\Gamma\left(l+\frac{3}{2}\right)2^{l+\frac{1}{2}}}m_p(m \omega_{\rm orb})^{l+\frac{1}{2}}  Y_l^m\left(\frac{\pi}{2},0\right)\sqrt{1-(r_{\rm orb} \omega_{\rm orb})^2}\nn\\
& \frac{\phi^I}{r_{\rm orb}} \left[ \frac{e^{-i m \omega_{\rm orb} t}-e^{-i\text{sign}(m) \omega_{n'} t}}{W(m\omega_{\rm orb})}\right] \,,\nonumber
\end{align}
%
again with $\phi^I=\phi^I(r_{\rm orb}; m \omega_{\rm orb})$. 
So, in this case, the energy density at the origin is
%
\begin{equation}
T_{t t}(r\to 0)\sim \left|\frac{e^{-i \omega_{\rm orb} t}-e^{-i\omega_{n'} t}}{W(\omega_{\rm orb})}\right|^2\frac{\omega_{\rm orb}^3}{16 \pi^3}\left(\frac{m_p \phi^I}{r_{\rm orb}}\right)^2\left[1-\left(r_{\rm orb} \omega_{\rm orb}\right)^2\right]\,.\nonumber
\end{equation}
%
Notice that, with this choice of coefficients $A_{l,n}^m$, the energy density $T_{t t}(r\to 0)$ is well-defined in the limit $\omega_{\rm orb}\to \omega_{n'}$, and is equal to
%
\begin{equation}
\lim_{\omega_{\rm orb}\to \omega_{n'}} T_{t t}(r\to 0)\sim \frac{t^2}{\left[W'(\omega_{n'})\right]^2}\frac{\omega_{n'}^3}{16 \pi^3}\left(\frac{m_p \phi^I(r_{\rm orb};\omega_{n'})}{r_{\rm orb}}\right)^2\left[1-\left(r_{\rm orb} \omega_{n'}\right)^2\right]\,,\nonumber
\end{equation}
%
where $W'(\omega)$ is the Wronskian derivative with respect to the frequency. Thus, one concludes that in a resonance the energy density at the origin increases quadratically with time.


==> app_vectorizedTools.tex <==


